On Stochastic Rewriting and Combinatorics via Rule-Algebraic Methods

Building upon the rule-algebraic stochastic mechanics framework, we present new results on the relationship of stochastic rewriting systems described in terms of continuous-time Markov chains, their embedded discrete-time Markov chains and certain types of generating function expressions in combinatorics. We introduce a number of generating function techniques that permit a novel form of static analysis for rewriting systems based upon marginalizing distributions over the states of the rewriting systems via pattern-counting observables.

==> eptcsdata.tex <==
\providecommand{\firstpage}{11}
\providecommand{\publicationstatus}{P. Bahr (Ed.): 11th International Workshop on\\
Computing with Terms and Graphs (TERMGRAPH 2020)\\
EPTCS 334, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.334.2}{10.4204/EPTCS.334.2}}
\pdfoutput=1

